Fair Division with Interdependent Values

We introduce the study of designing allocation mechanisms for fairly allocating indivisible goods in settings with interdependent valuation functions. In our setting, there is a set of goods that needs to be allocated to a set of agents (without disposal). Each agent is given a private signal, and his valuation function depends on the signals of all agents. Without the use of payments, there are strong impossibility results for designing strategyproof allocation mechanisms even in settings without interdependent values. Therefore, we turn to design mechanisms that always admit equilibria that are fair with respect to their true signals, despite their potentially distorted perception. To do so, we first extend the definitions of pure Nash equilibrium and well-studied fairness notions in literature to the interdependent setting. We devise simple allocation mechanisms that always admit a fair equilibrium with respect to the true signals. We complement this result by showing that, even for very simple cases with binary additive interdependent valuation functions, no allocation mechanism that always admits an equilibrium, can guarantee that all equilibria are fair with respect to the true signals.

==> sections/impossibility.tex <==
\section{Impossibility results for IDV mechanisms} \label{sec:impossibility}

\subsection{One agent bids}
In this subsection, we have that $\bv_i = \bs_1, \forall i \in [n]$, and moreover all agents but the first one cannot express a bid. 
\begin{theorem}[Informal]
For any fairness notion, there is no IDV mechanism all of equilibria of which are fair, even in the case of 2 agents with dichotomous signals.
\end{theorem}

\begin{theorem}[Informal]
For the EFX (and thus MMS) fairness notion, there is no IDV mechanism that has at least one fair equilibrium, even in the case of 2 agents with additive signals.
\end{theorem}

\subsection{Two asymmetric agents}
In this subsection, we have that $\bv_1 = \bs_1, \bv_2 \leq (1 + \beta) \bs_2$ (imagine something like $\bv_2 = \bs_2 + \beta \min(\bs_1, \bs_2)$), and both agents can express a bid. We want to show that $\forall \beta > 0$, there is no IDV mechanism with the following restrictions that has at least one fair equilibrium: (1) it always produces a complete allocation, (2) agent $i$ can only declare $b(\bs_i) = \bb_i$, where $b: \R^{2^{[m]}} \rightarrow \R^{2^{[m]}}$ (the agent declares something about her signal only, and nobody else's).

==> sections/mms.tex <==
\section{MMS Mechanisms with Interdependent Values} \label{sec:idv-mms}

The theorem that follows holds under the following assumptions: (1) 2 agents, (2) additive valuations, (3) they have the same valuation $\bv_1 = \bs_1 = \bv_2$ (for this case equal to the first agent's), and (4) both agents submit a bid.
\begin{theorem}
    There exists a mechanism (Generalized Cut-\&-Choose) that always has an equilibrium that corresponds to an MMS allocation according to the true signals of the agents.
\end{theorem}

==> sections/model.tex <==
\section{Model}

We study the problem of dividing $m$ indivisible items among $n$ strategic agents. Each agent $i \in [n]$ has
\begin{itemize}
    \item A private signal $s_{iT}, \forall T \subseteq [m]$.
    \item A public valuation function $v_{iT}(\bs_{T})$, where $\bs_T = (s_{iT})_{i \in [n]} \in \R^n_{\geq 0}$ is the vector of signals each agent has on set $T$. For conciseness, we denote by $\bs$ the set of all signals $\{\bs_T\}_{T \in 2^{[m]}}$.
    \item A different representation of the above is given by the (exponentially-sized) matrix  of signals $\bS = (s_{iT}) \in \R^{n\times 2^{m}}_{\geq 0}$. 
\end{itemize}

We now define what a fair allocation and equilibrium mean in this setting. Informally, we would like to have that the allocation a mechanism produces is fair according to the true matrix of signals $\bS$ and not the declared one $\bS^\prime$: i.e., if the fairness notion is $\text{FAIR} \in \{\text{EF1}, \text{EFX}, \text{MMS}, \ldots\}$, then the allocation is $\text{FAIR}_{\bS}$ (and not necessarily $\text{FAIR}_{\bS^\prime}$). In addition, we would like declaration $\bS^\prime$ to be a PNE, so that no agent is incentivized to deviate from this (potentially) untruthful declaration.

\begin{definition}[Fair-signal Allocation]\label{def:fair-alloc}
    Consider a setting with $n$ agents and $m$ items, with true matrix of signals $\bS$. We say that the partition of items to agents $\cA = \{A_1, \ldots, A_n\}$ is a fair-signal allocation, denoted by $\text{FAIR}_{\bS}$, if it is $\text{FAIR}$ with respect to $v_{iA_k}(\bs_{A_k})$, for all $i, k \in [n]$.
\end{definition}

\begin{definition}[Fair-signal Equilibrium]\label{def:fair-eq}
    Consider a setting with $n$ agents and $m$ items, with true matrix of signals $\bS$ and declared matrix of signals $\bS^\prime$. We say that the partition of items to agents $\cA = \{A_1, \ldots, A_n\}$ is a fair-signal equilibrium if
    \begin{enumerate}
        \item $\cA$ is $\text{FAIR}_{\bS}$, i.e., it is a fair-signal allocation according to the true matrix of signals $\bS$;
        \item For all signal matrices $\bS^{\prime\prime} \neq \bS^\prime$, $\forall i \in [n], v_{iA^\prime_i}(s_{iA^\prime_i}, \bs_{-iA^\prime_{-i}}) \geq v_{iA^{\prime\prime}_i}(s_{iA^{\prime\prime}_i}, \bs_{-iA^{\prime\prime}_{-i}})$, i.e., no agent $i$ can improve her utility by declaring a signal vector $\bs_i^{\prime\prime}$ different from $\bs_i^{\prime}$.
    \end{enumerate}
\end{definition}

\noindent The \textbf{guiding question} is, therefore,
\begin{center}
    \emph{Under what notions of fairness, and under what conditions on the agents' valuations as functions of the signals, does there exist a mechanism inducing fair-signal equilibria?}
\end{center}

\paragraph{Additive valuations.} Our central focus is on additive valuation functions, one of the most widely used classes of valuations: the value an agent attributes to a set of items is simply the sum of the value the agent attributes to each item belonging to that set. To this end, it is useful to explicitly define the value an agent has for a singleton $\{j\}$. Namely, $v_{i\{j\}}(\bs_{\{j\}}) = v_{ij}(s_{1j}, \ldots, s_{nj})$. Then, we have that the (additive) valuation function of agent $i$ for set of items $T$ is
\[
    v_{iT}(\bs_T) = \sum_{j \in T} v_{ij}(s_{1j}, \ldots, s_{nj}).
\]
Note how we can reduce the matrix of signals to be succinctly represented by $\bS = (s_{ij}) \in \R^{n\times m}_{\geq 0}$, where each agent simply has a signal for each item (as opposed to each subset of items).

==> sections/related.tex <==
\section{Related Work on Interdependent Mechanism Design with Money} \label{sec:related}

As previously underlined, mechanism design (with or without money) has traditionally been conceived for settings where agents' valuations are assumed to be independent. In this setting, a celebrated result by \citet{vickrey1961, Clarke1971, Groves1973} (the VCG mechanism) resolves the problem of truthful mechanism design optimally. However, the independence assumption falls short of characterizing natural scenarios, such as the illustrative oil drilling auction example of \citet{Wilson69}.  The auctioned land's value depends on how much oil there is underneath, and different agents might have different pieces of information (signals) about it. Most importantly, unlike traditional settings, each agent's value for that parcel of land depends on \emph{all} such pieces of information. In the context of single-item auctions, \citet{MilgromW82} formulated the \emph{interdependent value} (IDV) model, which prescribes each agent $i$ has a \emph{private} signal $s_i$ that summarizes the information she possesses about the item being auctioned. Furthermore, the value agent $i$ attributes to the item is a function of all signals, i.e., $v_i(s_i, s_{-i})$.

In the IDV model, it is impossible to design dominant strategy incentive-compatible mechanisms for single-item auctions in that if one agent does not report her signal truthfully, then another agent might not even be aware of its true valuation. More strongly, it is even impossible\footnote{\citet{JehielM01} show this impossibility even for Bayesian settings.} to design ex-post incentive compatible mechanisms \citep{JehielM01}, unless a condition called \emph{single-crossing} is met \citep{RoughgardenT13}. This signifies that each agent values her own signal above everybody else's. Beyond not being realistic, the single-crossing condition does not generalize well to multi-dimensional signal settings: \citet{EdenFFG18, EdenFTZ21, EdenGZ22}, and especially \citet{EdenFFGK19}, circumvent this issue (and later refined by \citet{LuSZ22}), extending ex-post incentive compatibility results to settings where valuations satisfy \emph{Submodularity over Signals} (SOS), a natural property to impose on valuations. Loosely, this means that the marginal increase in one's value due to her signal's increase is smaller the higher everybody else's signal is. Beyond auctions, some recent attention has been devolved to the setting of public projects, where diverse results have been attained \citep{CohenFMT23}.
